Simpler is Faster: Practical Distance Reporting by Sorting Along a Space-Filling Curve

Range reporting is a classical problem in computational geometry. A (rectangular) reporting data structure stores a point set $P$, such that, given a (rectangular) query region $\Delta$, it returns all points in $P \cap \Delta$. A variety of data structures support such queries with differing asymptotic guarantees such as k-d trees, range trees, R-trees, and quadtrees. A common variant of range queries are distance reporting queries, where the input is a query point $q$ and a radius $\delta$, and the goal is to report all points in $P$ within distance $\delta$ of $q$. Such queries frequently arise as subroutines in geometric data structures. Practical implementations typically answer distance queries through rectangular range queries using the data structures listed before. This paper revisits a simple and practical heuristic for distance reporting, originally proposed in TCS'97: sort the input point set~$P$ along a space-filling curve. Queries then reduce to scanning at most four contiguous ranges along the sorted curve. The fact that sorting along a space-filling curve is beneficial for range reporting is well-known. Many implementations use this technique to speed up their query and construction times. The point that this paper makes is subtle, but interesting: we argue that often, it is the space-filling curve rather than the overall data structure that provides the performance benefits. Thus, we offer a simple but effective alternative: only sort $P$ along a space-filling curve instead. We compare this approach to eight range searching implementations, across an elaborate test suite of real-world and synthetic data. Our experiments confirm this simple 200-line code approach out-performs all high-end implementations in terms of space usage and construction time. It presents almost always the best query times. In a dynamic setting, our approach dominates in performance.

==> Figures/experiments/const_realworld32_table_0_all.core.tex <==
athens\_large.out.uint32\_2&\numprint{1000000}&0.00&0.00&0.00&\bfseries 0.00&0.00&0.00\\
athens\_small.out.uint32\_2&\numprint{1000000}&0.00&0.00&0.00&\bfseries 0.00&0.00&0.00\\
berlin\_large.out.uint32\_2&\numprint{1000000}&0.02&0.02&0.02&\bfseries 0.02&0.03&0.04\\
chicago.out.uint32\_2&\numprint{1000000}&0.01&0.01&0.01&\bfseries 0.01&0.01&0.02\\
drifter.out.uint32\_2&\numprint{1000000}&0.04&0.04&0.05&\bfseries 0.03&0.05&0.05\\
tiger2006east.data.uint32\_2&\numprint{1000000}&0.64&0.64&0.64&\bfseries 0.42&0.64&0.83\\
tiger2006se.data.uint32\_2&\numprint{1000000}&\bfseries 0.00&0.00&0.00&0.00&0.00&0.00\\
unid\_00.out.uint32\_2&\numprint{1000000}&0.02&0.02&0.02&\bfseries 0.01&0.02&0.03\\


==> Figures/experiments/const_realworld32_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&hcds&hcds\_hilbert&pkd\\
athens\_large.out.uint32\_2&\numprint{1000000}&0.00&0.00&0.00&\bfseries 0.00&0.00&0.00\\
athens\_small.out.uint32\_2&\numprint{1000000}&0.00&0.00&0.00&\bfseries 0.00&0.00&0.00\\
berlin\_large.out.uint32\_2&\numprint{1000000}&0.02&0.02&0.02&\bfseries 0.02&0.03&0.04\\
chicago.out.uint32\_2&\numprint{1000000}&0.01&0.01&0.01&\bfseries 0.01&0.01&0.02\\
drifter.out.uint32\_2&\numprint{1000000}&0.04&0.04&0.05&\bfseries 0.03&0.05&0.05\\
tiger2006east.data.uint32\_2&\numprint{1000000}&0.64&0.64&0.64&\bfseries 0.42&0.64&0.83\\
tiger2006se.data.uint32\_2&\numprint{1000000}&\bfseries 0.00&0.00&0.00&0.00&0.00&0.00\\
unid\_00.out.uint32\_2&\numprint{1000000}&0.02&0.02&0.02&\bfseries 0.01&0.02&0.03\\

\end{longtblr}

==> Figures/experiments/const_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
athens\_large.out.uint32&0.008&0.008&0.007&0.010&0.012&\bfseries 0.005&0.009&0.070&0.013\\
athens\_small.out.uint32&2.282457e-04&2.329400e-04&2.298790e-04&0.002&0.002&\bfseries 1.755850e-04&3.198990e-04&0.002&0.001\\
berlin\_large.out.uint32&0.023&0.023&0.024&0.023&0.032&\bfseries 0.015&0.025&0.082&0.043\\
chicago.out.uint32&0.014&0.014&0.014&0.014&0.020&\bfseries 0.010&0.016&0.122&0.024\\
drifter.out.uint32&0.187&0.190&0.191&0.192&0.275&\bfseries 0.119&0.207&2.190&0.169\\
tiger2006east.data.uint32&2.544&2.565&2.533&1.768&2.550&\bfseries 1.618&2.423&24.951&2.757\\
tiger2006se.data.uint32&5.279&5.253&5.239&3.638&5.145&\bfseries 3.394&5.064&51.696&4.912\\
unid\_00.out.uint32&0.020&0.020&0.020&0.021&0.030&\bfseries 0.013&0.023&0.207&0.029\\

\end{longtblr}

==> Figures/experiments/construction_duration_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.001&0.001&0.001&0.004&0.004&\bfseries 8.044973e-04&0.001&0.009&0.003\\
$10^{5}$&0.014&0.014&0.014&0.014&0.019&\bfseries 0.009&0.014&0.115&0.031\\
$10^{6}$&0.167&0.168&0.167&0.188&0.234&\bfseries 0.107&0.158&1.339&0.237\\
$10^{7}$&2.030&2.039&2.032&1.410&1.859&\bfseries 1.272&1.765&15.280&3.582\\
$10^{8}$&23.808&23.486&23.530&14.691&19.089&\bfseries 13.932&18.909&&31.445\\
$10^{9}$&278.262&287.905&278.497&165.838&208.411&\bfseries 157.403&209.523&&420.476\\

\end{longtblr}

==> Figures/experiments/memper_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{6}$&69.724&69.682&69.817&69.007&68.823&\bfseries 66.022&66.057&784.140&68.768\\
$10^{7}$&513.051&515.435&512.322&440.435&441.267&\bfseries 386.999&397.084&8770.376&441.507\\
$10^{8}$&5045.823&5045.052&5045.566&\bfseries 3920.887&3921.172&3921.281&3921.199&&4176.385\\
$10^{9}$&50360.043&50359.879&50366.320&\bfseries 38679.059&38679.418&38679.379&38679.116&&41684.934\\

\end{longtblr}

==> Figures/experiments/prelim_const_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.176&\em OOT&4.327&0.115&0.159&\bfseries 0.095\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.177&\em OOT&4.337&0.111&0.164&\bfseries 0.100\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.178&\em OOT&4.328&0.111&0.162&\bfseries 0.099\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.178&\em OOT&4.343&0.113&0.160&\bfseries 0.099\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.179&\em OOT&4.349&0.113&0.164&\bfseries 0.096\\

\end{longtblr}

==> Figures/experiments/prelim_query_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.006&\em OOT&2.402&\bfseries 6.530e-04&6.983e-04&1.458\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.006&\em OOT&2.479&\bfseries 6.284e-04&8.522e-04&1.960\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.004&\em OOT&2.416&\bfseries 5.957e-04&8.302e-04&1.663\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.006&\em OOT&2.412&\bfseries 6.524e-04&7.616e-04&1.599\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.003&\em OOT&2.406&\bfseries 6.890e-04&7.300e-04&2.177\\

\end{longtblr}

==> Figures/experiments/prelim_table_0_all.core.tex <==
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.182&\em OOT&6.729&\bfseries 0.116&0.160&1.554\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.183&\em OOT&6.816&\bfseries 0.111&0.165&2.060\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.182&\em OOT&6.743&\bfseries 0.111&0.163&1.762\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.184&\em OOT&6.755&\bfseries 0.113&0.161&1.698\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.182&\em OOT&6.756&\bfseries 0.114&0.164&2.273\\


==> Figures/experiments/prelim_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.182&\em OOT&6.729&\bfseries 0.116&0.160&1.554\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.183&\em OOT&6.816&\bfseries 0.111&0.165&2.060\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.182&\em OOT&6.743&\bfseries 0.111&0.163&1.762\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.184&\em OOT&6.755&\bfseries 0.113&0.161&1.698\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.182&\em OOT&6.756&\bfseries 0.114&0.164&2.273\\

\end{longtblr}

==> Figures/experiments/query_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lllrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
0.001&athens\_large.out.uint32&norm&0.015&0.015&0.014&\bfseries 0.004&0.005&0.035&0.084&0.549&0.087\\
0.001&athens\_large.out.uint32&skew&0.053&0.048&0.050&\bfseries 0.015&0.016&0.048&0.097&0.369&0.294\\
0.001&athens\_large.out.uint32&unif&0.031&0.029&0.029&\bfseries 0.008&0.009&0.037&0.090&0.336&0.154\\
0.001&athens\_small.out.uint32&norm&0.029&0.027&0.027&\bfseries 0.008&0.011&0.042&0.086&0.105&0.107\\
0.001&athens\_small.out.uint32&skew&0.047&0.045&0.045&\bfseries 0.009&0.013&0.032&0.087&0.132&0.202\\
0.001&athens\_small.out.uint32&unif&0.039&0.038&0.037&\bfseries 0.008&0.010&0.042&0.087&0.131&0.140\\
0.001&berlin\_large.out.uint32&norm&0.035&0.034&0.033&\bfseries 0.014&0.018&0.043&0.099&0.299&0.158\\
0.001&berlin\_large.out.uint32&skew&0.134&0.130&0.131&\bfseries 0.058&0.069&0.090&0.140&0.730&0.468\\
0.001&berlin\_large.out.uint32&unif&0.081&0.081&0.081&\bfseries 0.036&0.041&0.064&0.115&0.711&0.287\\
0.001&chicago.out.uint32&norm&0.016&0.015&0.015&\bfseries 0.006&0.007&0.041&0.092&0.614&0.076\\
0.001&chicago.out.uint32&skew&0.085&0.087&0.082&\bfseries 0.031&0.036&0.070&0.118&0.924&0.380\\
0.001&chicago.out.uint32&unif&0.042&0.042&0.041&\bfseries 0.015&0.018&0.050&0.102&0.815&0.180\\
0.001&drifter.out.uint32&norm&0.013&0.014&0.017&\bfseries 0.009&0.010&0.060&0.104&0.924&0.064\\
0.001&drifter.out.uint32&skew&0.135&0.134&0.125&0.086&\bfseries 0.082&0.119&0.180&2.738&0.452\\
0.001&drifter.out.uint32&unif&0.100&0.104&0.107&0.064&\bfseries 0.063&0.115&0.153&2.653&0.304\\
0.001&tiger2006east.data.uint32&norm&0.167&0.206&0.165&0.179&\bfseries 0.145&0.230&0.263&10.909&0.819\\
0.001&tiger2006east.data.uint32&skew&0.234&0.273&0.262&0.225&\bfseries 0.197&0.267&0.331&13.212&1.204\\
0.001&tiger2006east.data.uint32&unif&0.250&0.245&0.245&0.255&\bfseries 0.232&0.320&0.360&14.246&1.217\\
0.001&tiger2006se.data.uint32&norm&0.111&0.101&0.102&\bfseries 0.021&0.022&0.068&0.119&18.103&0.053\\
0.001&tiger2006se.data.uint32&skew&0.919&\bfseries 0.564&0.573&1.236&1.145&1.442&1.554&22.461&29.487\\
0.001&tiger2006se.data.uint32&unif&0.296&\bfseries 0.238&0.240&0.366&0.380&0.460&0.519&20.669&8.626\\
0.001&unid\_00.out.uint32&norm&0.060&0.059&0.058&\bfseries 0.033&0.038&0.066&0.116&0.963&0.272\\
0.001&unid\_00.out.uint32&skew&0.085&0.084&0.084&\bfseries 0.048&0.052&0.079&0.135&1.336&0.440\\
0.001&unid\_00.out.uint32&unif&0.056&0.053&0.053&\bfseries 0.029&0.032&0.068&0.117&1.287&0.268\\

\end{longtblr}

==> Figures/experiments/query_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.120&0.117&0.116&\bfseries 0.022&0.031&0.043&0.093&0.324&0.499\\
$10^{5}$&0.210&0.205&0.202&\bfseries 0.071&0.089&0.089&0.140&1.174&0.824\\
$10^{6}$&0.376&0.370&0.366&\bfseries 0.202&0.223&0.204&0.255&4.541&1.280\\
$10^{7}$&0.878&0.874&0.881&0.681&\bfseries 0.663&0.684&0.679&15.334&2.493\\
$10^{8}$&2.430&2.371&2.387&2.300&\bfseries 2.139&2.389&2.340&&7.654\\
$10^{9}$&10.978&\bfseries 10.977&11.523&12.733&11.870&14.153&14.051&&84.949\\

\end{longtblr}

==> Figures/experiments/query_scaling_by_factorw_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
1.000000e-07&0.458&0.462&0.440&\bfseries 0.078&0.124&0.114&0.323&6.112&1.475\\
1.000000e-06&0.458&0.452&0.446&\bfseries 0.080&0.114&0.114&0.279&6.455&1.475\\
1.000000e-05&0.461&0.453&0.446&\bfseries 0.088&0.121&0.122&0.267&7.729&1.474\\
1.000000e-04&0.501&0.498&0.497&\bfseries 0.188&0.231&0.199&0.324&10.914&1.547\\
0.001&0.868&0.873&0.852&0.692&\bfseries 0.681&0.696&0.725&15.860&2.555\\
0.010&6.751&\bfseries 6.699&6.766&9.145&8.216&9.849&9.765&42.430&80.707\\
0.020&18.593&\bfseries 18.365&18.470&31.612&28.553&34.773&34.740&93.195&581.535\\

\end{longtblr}

==> Figures/experiments/runtime_dynamic_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&hcds&hcds\_hilbert&hcds\_std\\
$10^{4}$&$10^{4}$&0.009&0.008&0.021&\bfseries 0.003&0.005&0.003\\
$10^{4}$&\numprint{15000}&0.010&0.010&0.022&\bfseries 0.003&0.005&0.004\\
$10^{4}$&$10^{5}$&0.034&0.027&0.034&\bfseries 0.012&0.017&0.013\\
$10^{5}$&$10^{5}$&0.344&0.159&0.245&\bfseries 0.038&0.054&0.070\\
$10^{5}$&\numprint{150000}&0.424&0.191&0.261&\bfseries 0.045&0.064&0.085\\
$10^{5}$&$10^{6}$&1.769&0.726&0.537&\bfseries 0.182&0.235&0.303\\
$10^{6}$&$10^{6}$&17.053&5.665&3.951&\bfseries 0.806&0.977&2.588\\
$10^{6}$&\numprint{1500000}&21.473&7.181&4.489&\bfseries 1.020&1.183&3.260\\
$10^{6}$&$10^{7}$&95.065&32.577&13.575&\bfseries 4.293&4.745&14.371\\
$10^{7}$&$10^{7}$&1375.712&253.148&99.312&\bfseries 23.067&24.434&111.824\\
$10^{7}$&\numprint{15000000}&1739.294&332.676&121.817&\bfseries 30.852&32.249&151.198\\
$10^{7}$&$10^{8}$&\em OOT&1649.575&490.485&\bfseries 162.034&163.242&896.422\\

\end{longtblr}

==> Figures/experiments/size_realworld32_table_0_all.core.tex <==
athens\_large.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}\\
athens\_small.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}\\
berlin\_large.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}\\
chicago.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}\\
drifter.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}\\
tiger2006east.data.uint32\_2&\numprint{1000000}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}\\
tiger2006se.data.uint32\_2&\numprint{1000000}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}\\
unid\_00.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}\\


==> Figures/experiments/size_realworld32_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&hcds&hcds\_hilbert&pkd\\
athens\_large.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}&\bfseries \numprint{1628}\\
athens\_small.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}&\bfseries \numprint{502010}\\
berlin\_large.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}&\bfseries \numprint{21471356}\\
chicago.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}&\bfseries \numprint{6506571}\\
drifter.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}&\bfseries \numprint{18509158}\\
tiger2006east.data.uint32\_2&\numprint{1000000}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}&\bfseries \numprint{251073320}\\
tiger2006se.data.uint32\_2&\numprint{1000000}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}&\bfseries \numprint{0}\\
unid\_00.out.uint32\_2&\numprint{1000000}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}&\bfseries \numprint{45299836}\\

\end{longtblr}

==> Figures/experiments/size_realworld_table_0_all.core.tex <==
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\


==> Figures/experiments/size_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pkd\\
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\

\end{longtblr}

==> Figures/experiments_skew/const_realworld_table_0_all.core.tex <==
athens\_large.out.uint32&0.008&0.008&0.007&0.010&0.012&\bfseries 0.005&0.009&0.070&0.013\\
athens\_small.out.uint32&2.282e-04&2.329e-04&2.299e-04&0.002&0.002&\bfseries 1.756e-04&3.199e-04&0.002&0.001\\
berlin\_large.out.uint32&0.023&0.023&0.024&0.023&0.032&\bfseries 0.015&0.025&0.082&0.043\\
chicago.out.uint32&0.014&0.014&0.014&0.014&0.020&\bfseries 0.010&0.016&0.122&0.024\\
drifter.out.uint32&0.187&0.190&0.191&0.192&0.275&\bfseries 0.119&0.207&2.190&0.169\\
tiger2006east.data.uint32&2.544&2.565&2.533&1.768&2.550&\bfseries 1.618&2.423&24.951&2.757\\
tiger2006se.data.uint32&5.279&5.253&5.239&3.638&5.145&\bfseries 3.394&5.064&51.696&4.912\\
unid\_00.out.uint32&0.020&0.020&0.020&0.021&0.030&\bfseries 0.013&0.023&0.207&0.029\\


==> Figures/experiments_skew/const_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
athens\_large.out.uint32&0.008&0.008&0.007&0.010&0.012&\bfseries 0.005&0.009&0.070&0.013\\
athens\_small.out.uint32&2.282e-04&2.329e-04&2.299e-04&0.002&0.002&\bfseries 1.756e-04&3.199e-04&0.002&0.001\\
berlin\_large.out.uint32&0.023&0.023&0.024&0.023&0.032&\bfseries 0.015&0.025&0.082&0.043\\
chicago.out.uint32&0.014&0.014&0.014&0.014&0.020&\bfseries 0.010&0.016&0.122&0.024\\
drifter.out.uint32&0.187&0.190&0.191&0.192&0.275&\bfseries 0.119&0.207&2.190&0.169\\
tiger2006east.data.uint32&2.544&2.565&2.533&1.768&2.550&\bfseries 1.618&2.423&24.951&2.757\\
tiger2006se.data.uint32&5.279&5.253&5.239&3.638&5.145&\bfseries 3.394&5.064&51.696&4.912\\
unid\_00.out.uint32&0.020&0.020&0.020&0.021&0.030&\bfseries 0.013&0.023&0.207&0.029\\

\end{longtblr}

==> Figures/experiments_skew/construction_duration_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.001&0.001&0.001&0.004&0.005&\bfseries 8.047e-04&0.001&0.010&0.002\\
$10^{5}$&0.014&0.014&0.014&0.015&0.020&\bfseries 0.009&0.014&0.115&0.031\\
$10^{6}$&0.168&0.168&0.169&0.198&0.244&\bfseries 0.109&0.159&1.369&0.239\\
$10^{7}$&2.061&2.057&2.067&1.435&1.871&\bfseries 1.283&1.780&15.633&3.625\\
$10^{8}$&23.804&23.739&23.767&14.872&19.305&\bfseries 14.248&19.176&\em OOM&31.882\\
$10^{9}$&276.187&276.093&276.312&164.772&208.486&\bfseries 158.643&208.309&\em OOM&414.898\\

\end{longtblr}

==> Figures/experiments_skew/memper_scaling0001_norm_unif_table_0_all.core.tex <==
$10^{6}$&74.208&72.080&73.384&65.725&66.085&71.676&73.397&783.891&\bfseries 64.842\\
$10^{7}$&512.834&513.321&513.646&440.786&441.011&\bfseries 381.522&414.967&8770.034&440.800\\
$10^{8}$&5043.552&5044.665&5044.665&\bfseries 3920.582&3920.715&3920.592&3920.589&\em OOM&4175.066\\
$10^{9}$&50363.837&50364.306&50365.993&\bfseries 38681.833&38682.031&38681.946&38681.892&\em OOM&41674.538\\


==> Figures/experiments_skew/memper_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{6}$&74.208&72.080&73.384&65.725&66.085&71.676&73.397&783.891&\bfseries 64.842\\
$10^{7}$&512.834&513.321&513.646&440.786&441.011&\bfseries 381.522&414.967&8770.034&440.800\\
$10^{8}$&5043.552&5044.665&5044.665&\bfseries 3920.582&3920.715&3920.592&3920.589&\em OOM&4175.066\\
$10^{9}$&50363.837&50364.306&50365.993&\bfseries 38681.833&38682.031&38681.946&38681.892&\em OOM&41674.538\\

\end{longtblr}

==> Figures/experiments_skew/prelim_const_table_0_all.core.tex <==
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.176&\em OOT&4.327&0.115&0.159&\bfseries 0.095\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.177&\em OOT&4.337&0.111&0.164&\bfseries 0.100\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.178&\em OOT&4.328&0.111&0.162&\bfseries 0.099\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.178&\em OOT&4.343&0.113&0.160&\bfseries 0.099\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.179&\em OOT&4.349&0.113&0.164&\bfseries 0.096\\


==> Figures/experiments_skew/prelim_const_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.176&\em OOT&4.327&0.115&0.159&\bfseries 0.095\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.177&\em OOT&4.337&0.111&0.164&\bfseries 0.100\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.178&\em OOT&4.328&0.111&0.162&\bfseries 0.099\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.178&\em OOT&4.343&0.113&0.160&\bfseries 0.099\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.179&\em OOT&4.349&0.113&0.164&\bfseries 0.096\\

\end{longtblr}

==> Figures/experiments_skew/prelim_query_table_0_all.core.tex <==
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.006&\em OOT&2.402&\bfseries 6.530e-04&6.983e-04&1.458\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.006&\em OOT&2.479&\bfseries 6.284e-04&8.522e-04&1.960\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.004&\em OOT&2.416&\bfseries 5.957e-04&8.302e-04&1.663\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.006&\em OOT&2.412&\bfseries 6.524e-04&7.616e-04&1.599\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.003&\em OOT&2.406&\bfseries 6.890e-04&7.300e-04&2.177\\


==> Figures/experiments_skew/prelim_query_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.006&\em OOT&2.402&\bfseries 6.530e-04&6.983e-04&1.458\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.006&\em OOT&2.479&\bfseries 6.284e-04&8.522e-04&1.960\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.004&\em OOT&2.416&\bfseries 5.957e-04&8.302e-04&1.663\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.006&\em OOT&2.412&\bfseries 6.524e-04&7.616e-04&1.599\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.003&\em OOT&2.406&\bfseries 6.890e-04&7.300e-04&2.177\\

\end{longtblr}

==> Figures/experiments_skew/query_realworld_table_0_all.core.tex <==
0.001&athens\_large.out.uint32&norm&0.015&0.015&0.014&\bfseries 0.004&0.005&0.035&0.084&0.549&0.087\\
0.001&athens\_large.out.uint32&skew&0.053&0.048&0.050&\bfseries 0.015&0.016&0.048&0.097&0.369&0.294\\
0.001&athens\_large.out.uint32&unif&0.031&0.029&0.029&\bfseries 0.008&0.009&0.037&0.090&0.336&0.154\\
0.001&athens\_small.out.uint32&norm&0.029&0.027&0.027&\bfseries 0.008&0.011&0.042&0.086&0.105&0.107\\
0.001&athens\_small.out.uint32&skew&0.047&0.045&0.045&\bfseries 0.009&0.013&0.032&0.087&0.132&0.202\\
0.001&athens\_small.out.uint32&unif&0.039&0.038&0.037&\bfseries 0.008&0.010&0.042&0.087&0.131&0.140\\
0.001&berlin\_large.out.uint32&norm&0.035&0.034&0.033&\bfseries 0.014&0.018&0.043&0.099&0.299&0.158\\
0.001&berlin\_large.out.uint32&skew&0.134&0.130&0.131&\bfseries 0.058&0.069&0.090&0.140&0.730&0.468\\
0.001&berlin\_large.out.uint32&unif&0.081&0.081&0.081&\bfseries 0.036&0.041&0.064&0.115&0.711&0.287\\
0.001&chicago.out.uint32&norm&0.016&0.015&0.015&\bfseries 0.006&0.007&0.041&0.092&0.614&0.076\\
0.001&chicago.out.uint32&skew&0.085&0.087&0.082&\bfseries 0.031&0.036&0.070&0.118&0.924&0.380\\
0.001&chicago.out.uint32&unif&0.042&0.042&0.041&\bfseries 0.015&0.018&0.050&0.102&0.815&0.180\\
0.001&drifter.out.uint32&norm&0.013&0.014&0.017&\bfseries 0.009&0.010&0.060&0.104&0.924&0.064\\
0.001&drifter.out.uint32&skew&0.135&0.134&0.125&0.086&\bfseries 0.082&0.119&0.180&2.738&0.452\\
0.001&drifter.out.uint32&unif&0.100&0.104&0.107&0.064&\bfseries 0.063&0.115&0.153&2.653&0.304\\
0.001&tiger2006east.data.uint32&norm&0.167&0.206&0.165&0.179&\bfseries 0.145&0.230&0.263&10.909&0.819\\
0.001&tiger2006east.data.uint32&skew&0.234&0.273&0.262&0.225&\bfseries 0.197&0.267&0.331&13.212&1.204\\
0.001&tiger2006east.data.uint32&unif&0.250&0.245&0.245&0.255&\bfseries 0.232&0.320&0.360&14.246&1.217\\
0.001&tiger2006se.data.uint32&norm&0.111&0.101&0.102&\bfseries 0.021&0.022&0.068&0.119&18.103&0.053\\
0.001&tiger2006se.data.uint32&skew&0.919&\bfseries 0.564&0.573&1.236&1.145&1.442&1.554&22.461&29.487\\
0.001&tiger2006se.data.uint32&unif&0.296&\bfseries 0.238&0.240&0.366&0.380&0.460&0.519&20.669&8.626\\
0.001&unid\_00.out.uint32&norm&0.060&0.059&0.058&\bfseries 0.033&0.038&0.066&0.116&0.963&0.272\\
0.001&unid\_00.out.uint32&skew&0.085&0.084&0.084&\bfseries 0.048&0.052&0.079&0.135&1.336&0.440\\
0.001&unid\_00.out.uint32&unif&0.056&0.053&0.053&\bfseries 0.029&0.032&0.068&0.117&1.287&0.268\\


==> Figures/experiments_skew/query_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lllrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
0.001&athens\_large.out.uint32&norm&0.015&0.015&0.014&\bfseries 0.004&0.005&0.035&0.084&0.549&0.087\\
0.001&athens\_large.out.uint32&skew&0.053&0.048&0.050&\bfseries 0.015&0.016&0.048&0.097&0.369&0.294\\
0.001&athens\_large.out.uint32&unif&0.031&0.029&0.029&\bfseries 0.008&0.009&0.037&0.090&0.336&0.154\\
0.001&athens\_small.out.uint32&norm&0.029&0.027&0.027&\bfseries 0.008&0.011&0.042&0.086&0.105&0.107\\
0.001&athens\_small.out.uint32&skew&0.047&0.045&0.045&\bfseries 0.009&0.013&0.032&0.087&0.132&0.202\\
0.001&athens\_small.out.uint32&unif&0.039&0.038&0.037&\bfseries 0.008&0.010&0.042&0.087&0.131&0.140\\
0.001&berlin\_large.out.uint32&norm&0.035&0.034&0.033&\bfseries 0.014&0.018&0.043&0.099&0.299&0.158\\
0.001&berlin\_large.out.uint32&skew&0.134&0.130&0.131&\bfseries 0.058&0.069&0.090&0.140&0.730&0.468\\
0.001&berlin\_large.out.uint32&unif&0.081&0.081&0.081&\bfseries 0.036&0.041&0.064&0.115&0.711&0.287\\
0.001&chicago.out.uint32&norm&0.016&0.015&0.015&\bfseries 0.006&0.007&0.041&0.092&0.614&0.076\\
0.001&chicago.out.uint32&skew&0.085&0.087&0.082&\bfseries 0.031&0.036&0.070&0.118&0.924&0.380\\
0.001&chicago.out.uint32&unif&0.042&0.042&0.041&\bfseries 0.015&0.018&0.050&0.102&0.815&0.180\\
0.001&drifter.out.uint32&norm&0.013&0.014&0.017&\bfseries 0.009&0.010&0.060&0.104&0.924&0.064\\
0.001&drifter.out.uint32&skew&0.135&0.134&0.125&0.086&\bfseries 0.082&0.119&0.180&2.738&0.452\\
0.001&drifter.out.uint32&unif&0.100&0.104&0.107&0.064&\bfseries 0.063&0.115&0.153&2.653&0.304\\
0.001&tiger2006east.data.uint32&norm&0.167&0.206&0.165&0.179&\bfseries 0.145&0.230&0.263&10.909&0.819\\
0.001&tiger2006east.data.uint32&skew&0.234&0.273&0.262&0.225&\bfseries 0.197&0.267&0.331&13.212&1.204\\
0.001&tiger2006east.data.uint32&unif&0.250&0.245&0.245&0.255&\bfseries 0.232&0.320&0.360&14.246&1.217\\
0.001&tiger2006se.data.uint32&norm&0.111&0.101&0.102&\bfseries 0.021&0.022&0.068&0.119&18.103&0.053\\
0.001&tiger2006se.data.uint32&skew&0.919&\bfseries 0.564&0.573&1.236&1.145&1.442&1.554&22.461&29.487\\
0.001&tiger2006se.data.uint32&unif&0.296&\bfseries 0.238&0.240&0.366&0.380&0.460&0.519&20.669&8.626\\
0.001&unid\_00.out.uint32&norm&0.060&0.059&0.058&\bfseries 0.033&0.038&0.066&0.116&0.963&0.272\\
0.001&unid\_00.out.uint32&skew&0.085&0.084&0.084&\bfseries 0.048&0.052&0.079&0.135&1.336&0.440\\
0.001&unid\_00.out.uint32&unif&0.056&0.053&0.053&\bfseries 0.029&0.032&0.068&0.117&1.287&0.268\\

\end{longtblr}

==> Figures/experiments_skew/query_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.162&0.158&0.157&\bfseries 0.028&0.042&0.044&0.097&0.408&0.649\\
$10^{5}$&0.262&0.255&0.258&\bfseries 0.093&0.120&0.102&0.153&1.520&0.982\\
$10^{6}$&0.448&0.441&0.446&0.295&0.321&\bfseries 0.291&0.327&6.433&1.516\\
$10^{7}$&1.013&1.036&1.021&0.913&\bfseries 0.882&0.890&0.893&19.246&3.025\\
$10^{8}$&2.849&2.806&2.778&2.810&\bfseries 2.553&2.833&2.675&\em OOM&8.347\\
$10^{9}$&11.186&10.955&\bfseries 10.853&13.980&12.454&14.744&14.288&\em OOM&68.678\\

\end{longtblr}

==> Figures/experiments_skew/query_scaling_by_factorw_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
1.000e-07&0.569&0.569&0.552&\bfseries 0.100&0.170&0.137&0.394&6.381&1.837\\
1.000e-06&0.562&0.559&0.568&\bfseries 0.102&0.155&0.141&0.352&6.869&1.828\\
1.000e-05&0.570&0.569&0.560&\bfseries 0.115&0.166&0.151&0.340&8.524&1.828\\
1.000e-04&0.635&0.617&0.612&0.253&0.328&\bfseries 0.248&0.422&13.497&1.923\\
0.001&1.051&1.033&1.018&0.960&\bfseries 0.936&0.938&0.989&20.196&3.191\\
0.010&6.657&6.672&\bfseries 6.649&9.188&8.104&9.770&9.756&42.819&81.108\\
0.020&18.407&\bfseries 18.304&18.633&31.807&28.406&34.642&34.419&94.418&570.746\\

\end{longtblr}

==> Figures/experiments_skew/size_realworld_table_0_all.core.tex <==
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\


==> Figures/experiments_skew/size_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pkd\\
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\

\end{longtblr}

==> Figures/experiments_unif/const_realworld_table_0_all.core.tex <==
athens\_large.out.uint32&0.008&0.008&0.007&0.010&0.012&\bfseries 0.005&0.009&0.070&0.013\\
athens\_small.out.uint32&2.282e-04&2.329e-04&2.299e-04&0.002&0.002&\bfseries 1.756e-04&3.199e-04&0.002&0.001\\
berlin\_large.out.uint32&0.023&0.023&0.024&0.023&0.032&\bfseries 0.015&0.025&0.082&0.043\\
chicago.out.uint32&0.014&0.014&0.014&0.014&0.020&\bfseries 0.010&0.016&0.122&0.024\\
drifter.out.uint32&0.187&0.190&0.191&0.192&0.275&\bfseries 0.119&0.207&2.190&0.169\\
tiger2006east.data.uint32&2.544&2.565&2.533&1.768&2.550&\bfseries 1.618&2.423&24.951&2.757\\
tiger2006se.data.uint32&5.279&5.253&5.239&3.638&5.145&\bfseries 3.394&5.064&51.696&4.912\\
unid\_00.out.uint32&0.020&0.020&0.020&0.021&0.030&\bfseries 0.013&0.023&0.207&0.029\\


==> Figures/experiments_unif/const_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
athens\_large.out.uint32&0.008&0.008&0.007&0.010&0.012&\bfseries 0.005&0.009&0.070&0.013\\
athens\_small.out.uint32&2.282e-04&2.329e-04&2.299e-04&0.002&0.002&\bfseries 1.756e-04&3.199e-04&0.002&0.001\\
berlin\_large.out.uint32&0.023&0.023&0.024&0.023&0.032&\bfseries 0.015&0.025&0.082&0.043\\
chicago.out.uint32&0.014&0.014&0.014&0.014&0.020&\bfseries 0.010&0.016&0.122&0.024\\
drifter.out.uint32&0.187&0.190&0.191&0.192&0.275&\bfseries 0.119&0.207&2.190&0.169\\
tiger2006east.data.uint32&2.544&2.565&2.533&1.768&2.550&\bfseries 1.618&2.423&24.951&2.757\\
tiger2006se.data.uint32&5.279&5.253&5.239&3.638&5.145&\bfseries 3.394&5.064&51.696&4.912\\
unid\_00.out.uint32&0.020&0.020&0.020&0.021&0.030&\bfseries 0.013&0.023&0.207&0.029\\

\end{longtblr}

==> Figures/experiments_unif/construction_duration_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.001&0.001&0.001&0.004&0.004&\bfseries 8.142e-04&0.001&0.009&0.002\\
$10^{5}$&0.014&0.014&0.014&0.015&0.020&\bfseries 0.009&0.014&0.115&0.031\\
$10^{6}$&0.168&0.167&0.168&0.206&0.249&\bfseries 0.108&0.159&1.376&0.239\\
$10^{7}$&2.063&2.061&2.052&1.423&1.859&\bfseries 1.279&1.784&15.725&3.634\\
$10^{8}$&23.732&23.658&23.676&14.894&19.327&\bfseries 14.270&19.225&\em OOM&31.904\\
$10^{9}$&274.948&275.382&275.193&164.830&208.450&\bfseries 158.713&207.996&\em OOM&415.579\\

\end{longtblr}

==> Figures/experiments_unif/memper_scaling0001_norm_unif_table_0_all.core.tex <==
$10^{6}$&69.213&69.240&69.697&65.810&65.809&65.928&66.293&783.662&\bfseries 64.748\\
$10^{7}$&515.204&513.783&511.768&441.778&440.462&\bfseries 397.980&403.876&8769.408&441.041\\
$10^{8}$&5046.791&5043.623&5047.009&3920.540&3920.611&3920.652&\bfseries 3920.522&\em OOM&4171.316\\
$10^{9}$&50366.334&50363.444&50363.683&38681.740&38681.800&38681.683&\bfseries 38681.646&\em OOM&41669.133\\


==> Figures/experiments_unif/memper_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{6}$&69.213&69.240&69.697&65.810&65.809&65.928&66.293&783.662&\bfseries 64.748\\
$10^{7}$&515.204&513.783&511.768&441.778&440.462&\bfseries 397.980&403.876&8769.408&441.041\\
$10^{8}$&5046.791&5043.623&5047.009&3920.540&3920.611&3920.652&\bfseries 3920.522&\em OOM&4171.316\\
$10^{9}$&50366.334&50363.444&50363.683&38681.740&38681.800&38681.683&\bfseries 38681.646&\em OOM&41669.133\\

\end{longtblr}

==> Figures/experiments_unif/prelim_const_table_0_all.core.tex <==
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.176&\em OOT&4.327&0.115&0.159&\bfseries 0.095\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.177&\em OOT&4.337&0.111&0.164&\bfseries 0.100\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.178&\em OOT&4.328&0.111&0.162&\bfseries 0.099\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.178&\em OOT&4.343&0.113&0.160&\bfseries 0.099\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.179&\em OOT&4.349&0.113&0.164&\bfseries 0.096\\


==> Figures/experiments_unif/prelim_const_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.176&\em OOT&4.327&0.115&0.159&\bfseries 0.095\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.177&\em OOT&4.337&0.111&0.164&\bfseries 0.100\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.178&\em OOT&4.328&0.111&0.162&\bfseries 0.099\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.178&\em OOT&4.343&0.113&0.160&\bfseries 0.099\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.179&\em OOT&4.349&0.113&0.164&\bfseries 0.096\\

\end{longtblr}

==> Figures/experiments_unif/prelim_query_table_0_all.core.tex <==
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.006&\em OOT&2.402&\bfseries 6.530e-04&6.983e-04&1.458\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.006&\em OOT&2.479&\bfseries 6.284e-04&8.522e-04&1.960\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.004&\em OOT&2.416&\bfseries 5.957e-04&8.302e-04&1.663\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.006&\em OOT&2.412&\bfseries 6.524e-04&7.616e-04&1.599\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.003&\em OOT&2.406&\bfseries 6.890e-04&7.300e-04&2.177\\


==> Figures/experiments_unif/prelim_query_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&cgal\_kd&cgal\_rt&hcds&hcds\_hilbert&pargeo\\
norm:1000000:unif:1000:4:0.001&\numprint{885}&0.006&\em OOT&2.402&\bfseries 6.530e-04&6.983e-04&1.458\\
norm:1000000:unif:1000:5:0.001&\numprint{922}&0.006&\em OOT&2.479&\bfseries 6.284e-04&8.522e-04&1.960\\
norm:1000000:unif:1000:2:0.001&\numprint{958}&0.004&\em OOT&2.416&\bfseries 5.957e-04&8.302e-04&1.663\\
norm:1000000:unif:1000:1:0.001&\numprint{992}&0.006&\em OOT&2.412&\bfseries 6.524e-04&7.616e-04&1.599\\
norm:1000000:unif:1000:3:0.001&\numprint{1061}&0.003&\em OOT&2.406&\bfseries 6.890e-04&7.300e-04&2.177\\

\end{longtblr}

==> Figures/experiments_unif/query_realworld_table_0_all.core.tex <==
0.001&athens\_large.out.uint32&norm&0.015&0.015&0.014&\bfseries 0.004&0.005&0.035&0.084&0.549&0.087\\
0.001&athens\_large.out.uint32&skew&0.053&0.048&0.050&\bfseries 0.015&0.016&0.048&0.097&0.369&0.294\\
0.001&athens\_large.out.uint32&unif&0.031&0.029&0.029&\bfseries 0.008&0.009&0.037&0.090&0.336&0.154\\
0.001&athens\_small.out.uint32&norm&0.029&0.027&0.027&\bfseries 0.008&0.011&0.042&0.086&0.105&0.107\\
0.001&athens\_small.out.uint32&skew&0.047&0.045&0.045&\bfseries 0.009&0.013&0.032&0.087&0.132&0.202\\
0.001&athens\_small.out.uint32&unif&0.039&0.038&0.037&\bfseries 0.008&0.010&0.042&0.087&0.131&0.140\\
0.001&berlin\_large.out.uint32&norm&0.035&0.034&0.033&\bfseries 0.014&0.018&0.043&0.099&0.299&0.158\\
0.001&berlin\_large.out.uint32&skew&0.134&0.130&0.131&\bfseries 0.058&0.069&0.090&0.140&0.730&0.468\\
0.001&berlin\_large.out.uint32&unif&0.081&0.081&0.081&\bfseries 0.036&0.041&0.064&0.115&0.711&0.287\\
0.001&chicago.out.uint32&norm&0.016&0.015&0.015&\bfseries 0.006&0.007&0.041&0.092&0.614&0.076\\
0.001&chicago.out.uint32&skew&0.085&0.087&0.082&\bfseries 0.031&0.036&0.070&0.118&0.924&0.380\\
0.001&chicago.out.uint32&unif&0.042&0.042&0.041&\bfseries 0.015&0.018&0.050&0.102&0.815&0.180\\
0.001&drifter.out.uint32&norm&0.013&0.014&0.017&\bfseries 0.009&0.010&0.060&0.104&0.924&0.064\\
0.001&drifter.out.uint32&skew&0.135&0.134&0.125&0.086&\bfseries 0.082&0.119&0.180&2.738&0.452\\
0.001&drifter.out.uint32&unif&0.100&0.104&0.107&0.064&\bfseries 0.063&0.115&0.153&2.653&0.304\\
0.001&tiger2006east.data.uint32&norm&0.167&0.206&0.165&0.179&\bfseries 0.145&0.230&0.263&10.909&0.819\\
0.001&tiger2006east.data.uint32&skew&0.234&0.273&0.262&0.225&\bfseries 0.197&0.267&0.331&13.212&1.204\\
0.001&tiger2006east.data.uint32&unif&0.250&0.245&0.245&0.255&\bfseries 0.232&0.320&0.360&14.246&1.217\\
0.001&tiger2006se.data.uint32&norm&0.111&0.101&0.102&\bfseries 0.021&0.022&0.068&0.119&18.103&0.053\\
0.001&tiger2006se.data.uint32&skew&0.919&\bfseries 0.564&0.573&1.236&1.145&1.442&1.554&22.461&29.487\\
0.001&tiger2006se.data.uint32&unif&0.296&\bfseries 0.238&0.240&0.366&0.380&0.460&0.519&20.669&8.626\\
0.001&unid\_00.out.uint32&norm&0.060&0.059&0.058&\bfseries 0.033&0.038&0.066&0.116&0.963&0.272\\
0.001&unid\_00.out.uint32&skew&0.085&0.084&0.084&\bfseries 0.048&0.052&0.079&0.135&1.336&0.440\\
0.001&unid\_00.out.uint32&unif&0.056&0.053&0.053&\bfseries 0.029&0.032&0.068&0.117&1.287&0.268\\


==> Figures/experiments_unif/query_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lllrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
0.001&athens\_large.out.uint32&norm&0.015&0.015&0.014&\bfseries 0.004&0.005&0.035&0.084&0.549&0.087\\
0.001&athens\_large.out.uint32&skew&0.053&0.048&0.050&\bfseries 0.015&0.016&0.048&0.097&0.369&0.294\\
0.001&athens\_large.out.uint32&unif&0.031&0.029&0.029&\bfseries 0.008&0.009&0.037&0.090&0.336&0.154\\
0.001&athens\_small.out.uint32&norm&0.029&0.027&0.027&\bfseries 0.008&0.011&0.042&0.086&0.105&0.107\\
0.001&athens\_small.out.uint32&skew&0.047&0.045&0.045&\bfseries 0.009&0.013&0.032&0.087&0.132&0.202\\
0.001&athens\_small.out.uint32&unif&0.039&0.038&0.037&\bfseries 0.008&0.010&0.042&0.087&0.131&0.140\\
0.001&berlin\_large.out.uint32&norm&0.035&0.034&0.033&\bfseries 0.014&0.018&0.043&0.099&0.299&0.158\\
0.001&berlin\_large.out.uint32&skew&0.134&0.130&0.131&\bfseries 0.058&0.069&0.090&0.140&0.730&0.468\\
0.001&berlin\_large.out.uint32&unif&0.081&0.081&0.081&\bfseries 0.036&0.041&0.064&0.115&0.711&0.287\\
0.001&chicago.out.uint32&norm&0.016&0.015&0.015&\bfseries 0.006&0.007&0.041&0.092&0.614&0.076\\
0.001&chicago.out.uint32&skew&0.085&0.087&0.082&\bfseries 0.031&0.036&0.070&0.118&0.924&0.380\\
0.001&chicago.out.uint32&unif&0.042&0.042&0.041&\bfseries 0.015&0.018&0.050&0.102&0.815&0.180\\
0.001&drifter.out.uint32&norm&0.013&0.014&0.017&\bfseries 0.009&0.010&0.060&0.104&0.924&0.064\\
0.001&drifter.out.uint32&skew&0.135&0.134&0.125&0.086&\bfseries 0.082&0.119&0.180&2.738&0.452\\
0.001&drifter.out.uint32&unif&0.100&0.104&0.107&0.064&\bfseries 0.063&0.115&0.153&2.653&0.304\\
0.001&tiger2006east.data.uint32&norm&0.167&0.206&0.165&0.179&\bfseries 0.145&0.230&0.263&10.909&0.819\\
0.001&tiger2006east.data.uint32&skew&0.234&0.273&0.262&0.225&\bfseries 0.197&0.267&0.331&13.212&1.204\\
0.001&tiger2006east.data.uint32&unif&0.250&0.245&0.245&0.255&\bfseries 0.232&0.320&0.360&14.246&1.217\\
0.001&tiger2006se.data.uint32&norm&0.111&0.101&0.102&\bfseries 0.021&0.022&0.068&0.119&18.103&0.053\\
0.001&tiger2006se.data.uint32&skew&0.919&\bfseries 0.564&0.573&1.236&1.145&1.442&1.554&22.461&29.487\\
0.001&tiger2006se.data.uint32&unif&0.296&\bfseries 0.238&0.240&0.366&0.380&0.460&0.519&20.669&8.626\\
0.001&unid\_00.out.uint32&norm&0.060&0.059&0.058&\bfseries 0.033&0.038&0.066&0.116&0.963&0.272\\
0.001&unid\_00.out.uint32&skew&0.085&0.084&0.084&\bfseries 0.048&0.052&0.079&0.135&1.336&0.440\\
0.001&unid\_00.out.uint32&unif&0.056&0.053&0.053&\bfseries 0.029&0.032&0.068&0.117&1.287&0.268\\

\end{longtblr}

==> Figures/experiments_unif/query_scaling0001_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
$10^{4}$&0.196&0.191&0.189&\bfseries 0.032&0.049&0.047&0.099&0.438&0.709\\
$10^{5}$&0.289&0.283&0.281&\bfseries 0.105&0.143&0.111&0.163&1.707&1.047\\
$10^{6}$&0.489&0.485&0.480&0.355&0.399&\bfseries 0.345&0.391&7.198&1.663\\
$10^{7}$&1.159&1.150&1.097&1.084&\bfseries 1.075&1.096&1.086&20.248&3.361\\
$10^{8}$&2.991&2.933&3.042&3.202&\bfseries 2.888&3.165&2.946&\em OOM&8.458\\
$10^{9}$&11.560&11.330&\bfseries 11.140&14.643&12.938&15.188&14.850&\em OOM&56.158\\

\end{longtblr}

==> Figures/experiments_unif/query_scaling_by_factorw_norm_unif_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {lrrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pam&pkd\\
1.000e-07&0.680&0.670&0.667&\bfseries 0.124&0.224&0.160&0.455&6.401&2.055\\
1.000e-06&0.669&0.672&0.657&\bfseries 0.126&0.203&0.164&0.406&6.911&2.064\\
1.000e-05&0.683&0.681&0.673&\bfseries 0.140&0.216&0.176&0.395&8.839&2.050\\
1.000e-04&0.750&0.740&0.723&0.308&0.415&\bfseries 0.289&0.495&14.005&2.169\\
0.001&1.167&1.168&1.127&1.140&\bfseries 1.112&1.118&1.135&20.815&3.554\\
0.010&6.716&6.751&\bfseries 6.584&9.246&8.208&9.801&9.726&42.891&81.201\\
0.020&\bfseries 18.413&18.518&18.535&31.900&28.539&34.692&34.604&94.350&576.249\\

\end{longtblr}

==> Figures/experiments_unif/size_realworld_table_0_all.core.tex <==
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\


==> Figures/experiments_unif/size_realworld_table_0_all.tex <==
\begin{longtblr}[
caption = {},
  label = {table:def},
 ]{
colspec = {llrrrrrrrr},rowhead =1, hlines,  row{even} = {gray9}, row{1} = {olive9},}
&runConfig\_shortName&boost\_lin&boost\_quad&boost\_star&ehcds&ehcds\_hilbert&hcds&hcds\_hilbert&pkd\\
athens\_large.out.uint32&$10^{6}$&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}&\bfseries \numprint{184147}\\
athens\_small.out.uint32&$10^{6}$&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}&\bfseries \numprint{403240}\\
berlin\_large.out.uint32&$10^{6}$&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}&\bfseries \numprint{2413405}\\
chicago.out.uint32&$10^{6}$&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}&\bfseries \numprint{571673}\\
drifter.out.uint32&$10^{6}$&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}&\bfseries \numprint{12807004}\\
tiger2006east.data.uint32&$10^{6}$&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}&\bfseries \numprint{1021323778}\\
tiger2006se.data.uint32&$10^{6}$&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}&\bfseries \numprint{62011}\\
unid\_00.out.uint32&$10^{6}$&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}&\bfseries \numprint{33015509}\\

\end{longtblr}
